Restricted Low-Rank Approximation via ADMM

The matrix low-rank approximation problem with additional convex constraints can find many applications and has been extensively studied before. However, this problem is shown to be nonconvex and NP-hard; most of the existing solutions are heuristic and application-dependent. In this paper, we show that, other than tons of application in current literature, this problem can be used to recover a feasible solution for SDP relaxation. By some sophisticated tricks, it can be equivalently posed in an appropriate form for the Alternating Direction Method of Multipliers (ADMM) to solve. The two updates of ADMM include the basic matrix low-rank approximation and projection onto a convex set. Different from the general non-convex problems, the sub-problems in each step of ADMM can be solved exactly and efficiently in spite of their non-convexity. Moreover, the algorithm will converge exponentially under proper conditions. The simulation results confirm its superiority over existing solutions. We believe that the results in this paper provide a useful tool for this important problem and will help to extend the application of ADMM to the non-convex regime.

==> theotherorder.tex <==
\subsubsection{The other update order}\label{sec:otherorder}
The previous analysis motivates the author to think about the other update order, \textit{i.e.}, to carry out $\mathbf{Y}$ update first and then $\mathbf{X}$ update. As we will show, the subproblems will not change much but the theoretical analysis will be simplified remarkably.

Under the same assumption that the dual variable $\mathbf{U}^k$ converges to $\bar{\mathbf{U}}$, by the same argument, $\mathbf{X}^k-\mathbf{Y}^k$ converges to 0 and the $\mathbf{Y}$ update can be denoted as
$$\mathbf{Y}^{k+1} = \underset{g(\mathbf{Y})\leq 0}{\text{argmin}}\|Y-(\bar{U}+\mathbf{Y}^k)\|_F^2,$$
which is a projection onto a convex set. We have the following corollary to characterize the convergence of primal variable.

\begin{corollary}\label{corollary:otherorder}
If we carry out $\mathbf{Y}$ update first, under the assumption that the dual variable converges, we can have
$$\|\mathbf{Y}^{k+2}-\mathbf{Y}^{k+1}\|_F\leq \|\mathbf{Y}^{k+1}-\mathbf{Y}^k\|_F.$$
\end{corollary}

This result is established by the fact that the projection onto a convex set is non-expansive.



